LEGO II: A 3 mm molecular line study covering 100 pc of one of the most actively star-forming portions within the Milky Way Disc

The current generation of (sub)mm-telescopes has allowed molecular line emission to become a major tool for studying the physical, kinematic, and chemical properties of extragalactic systems, yet exploiting these observations requires a detailed understanding of where emission lines originate within the Milky Way. In this paper, we present 60$^{\prime\prime}$ ($\sim$3pc) resolution observations of many 3mm-band molecular lines across a large map of the W49 massive star-forming region ($\sim$100$\times$100pc at 11kpc), which were taken as part of the "LEGO" IRAM-30m large project. We find that the spatial extent or brightness of the molecular line transitions are not well correlated with their critical densities, highlighting abundance and optical depth must be considered when estimating line emission characteristics. We explore how the total emission and emission efficiency (i.e. line brightness per H$_{2}$ column density) of the line emission vary as a function of molecular hydrogen column density and dust temperature. We find that there is not a single region of this parameter space responsible for the brightest and most efficiently emitting gas for all species. For example, we find that the HCN transition shows high emission efficiency at high column density ($10^{22}$cm$^{-2}$) and moderate temperatures (35K), whilst e.g. N$_2$H$^+$ emits most efficiently towards lower temperatures ($10^{22}$cm$^{-2}$; <20K). We determine $X_{\mathrm{CO} (1-0)} \sim 0.3 \times 10^{20} \mathrm{cm^{-2}(Kkms^{-1})^{-1}}$, and $\alpha_{\mathrm{HCN} (1-0)} \sim 30\mathrm{M_\odot(Kkms^{-1}pc^2)^{-1}}$, which both differ significantly from the commonly adopted values. In all, these results suggest caution should be taken when interpreting molecular line emission.

==> back_matter/references.tex <==
\bibliographystyle{./back_matter/mnras}

\bibliography{./back_matter/references} % if your bibtex file is called example.bib
%\bibliography{./back_matter/references} % if your bibtex file is called example.bib

